$K$-theoretic counterexamples to Ravenel's telescope conjecture

At each prime $p$ and height $n+1 \ge 2$, we prove that the telescopic and chromatic localizations of spectra differ. Specifically, for $\mathbb{Z}$ acting by Adams operations on $\mathrm{BP}\langle n \rangle$, we prove that the $T(n+1)$-localized algebraic $K$-theory of $\mathrm{BP}\langle n \rangle^{h\mathbb{Z}}$ is not $K(n+1)$-local. We also show that Galois hyperdescent, $\mathbb{A}^1$-invariance, and nil-invariance fail for the $K(n+1)$-localized algebraic $K$-theory of $K(n)$-local $\mathbb{E}_{\infty}$-rings. In the case $n=1$ and $p \ge 7$ we make complete computations of $T(2)_*\mathrm{K}(R)$, for $R$ certain finite Galois extensions of the $K(1)$-local sphere. We show for $p\geq 5$ that the algebraic $K$-theory of the $K(1)$-local sphere is asymptotically $L_2^{f}$-local.

==> split-descent.tex <==

In this subsection we prove a hyperdescent theorem for the $K$-theory of split extensions. We use this later by reducing hyperdescent to the split case.

\todo{rwb: I added a unipotence hypothesis here. I think it is necessary.}
\begin{dfn} \label{dfn:splitting}
  Let $\CC$ be a $p$-complete presentably symmetric monoidal stable category.
  Suppose we are given an $R \in \Alg(\CC^{B\Z,u})$.
  A \emph{splitting} of the $\Z$-action on $R$ 
  consists of a lift of $R$ to an 
  \[ \overline{R} \in \Alg_{\W (\LCF{\overrightarrow{\ZZ_p}})}(\CC^{B\Z,u}). \]
  Note this implies $R \in \Alg_{\W (\LCF{\overrightarrow{\ZZ_p}})}(\CC^{B\Z,u})$ since $\W (\LCF{\overrightarrow{\ZZ_p}}) \in \CC^{B\Z,u}$ \Cref{prop:unipotent_SW}, and $\CC^{B\Z,u}$ is closed under tensor products.
  We also introduce several variants of this definition:
  \begin{itemize}
  \item Given an $R \in \Alg(\Sp^{B\Z,u})$,
    a \emph{$T(n)$-local splitting} of the $\Z$-action on $R$
    is a splitting of the $\Z$-action on $L_{T(n)}R \in \Alg(\Sp_{T(n)}^{B\Z,u})$.
  \item Given an $R \in \Alg(\Sp^{B\Z,u})$ and an $A \in \CAlg(\Sp)$,
    we say that the $\Z$-action on $R$ is split by $A$
    if there is a splitting of the $\Z$-action on
    $ A \otimes R \in \Alg(\Mod(\Sp^{B\Z,u}; A))$.
  \item Given an $R \in \Alg(\Sp^{B\Z,u})$ and an $A \in \CAlg(\Sp)$,
    we say that the $\Z$-action on $R$ is $T(n)$-locally split by $A$
    if there is a splitting of the $\Z$-action on
    $L_{T(n)}(A \otimes R) \in \Alg(\Mod(\Sp_{T(n)}^{B\Z,u}; A))$. \qedhere
  \end{itemize}
\end{dfn}

\begin{rmk} \label{rmk:splitting-comm}
  In the commutative setting, given a splitting of $R \in \CAlg(\CC^{B\Z,u})$,
  by using the adjunction of \Cref{prop:witt-and-tilt},
  we can replace it with a commutative algebra map
  $\W (\LCF{\overrightarrow{\ZZ_p}})\to R$.
  Using this map, we learn that for any map $R \to S \in \CAlg(\CC^{B\Z,u})$,
  $S$ admits a splitting as well.
\end{rmk}
% \begin{lem} \label{rmk:splitting-comm}
%   For $R \in \CAlg(\CC^{B\Z,u})$, the space of splittings of $R$ are canonically equivalent to the set of maps $\LCF{\overrightarrow{\ZZ_p}} \to\pi_0^{\flat}R$.
% \end{lem}

% \begin{proof}
%     The space of splittings of $R$ is the same as the space of $\E_2$-maps $\W(LCF{\overrightarrow{\ZZ_p}})\to \mathcal{Z}_{\mathbb{E}_1}R$, where $\mathcal{Z}_{\mathbb{E}_1}R$ is the center of $R$ as an $\E_1$-algebra.
%     Given a splitting of $R$, we in particular have a unit map $\W(LCF{\overrightarrow{\ZZ_p}})\to R$. Applying $\pi_0^{\flat}$, we get an equivariant map $\LCF{\overrightarrow{\ZZ_p}} \to \pi_0^{\flat}R$, which we claim defines the equivalence. Indeed, the adjunction of \Cref{prop:witt-and-tilt} shows that this map is surjective on connected components, so it suffices to show that each fiber is contractible.

%     For a map $a:\LCF{\overrightarrow{\ZZ_p}} \to \pi_0^{\flat}R$ one can produce a contracting homotopy of the space of splittings lifting this by observing that the diagram
% \begin{center}
%         \begin{tikzcd}
%         \ar[r]\ar[d,"\epsilon"] \W(\LCF{\overrightarrow{\ZZ_p}}) & Z_{\E_2}R\ar[d,equal]\\
%         \W(\LCF{\overrightarrow{\ZZ_p}})\ar[r] & Z_{\E_2}R
%     \end{tikzcd}
% \end{center}
%   % to read off that
%   % \begin{itemize}
%   % \item $R$ is split if and only if
%   %   there is a $\Z$-equivariant map \todo{there is an issue with centrality for one of the implications (it's still true though)}$\LCF{\overrightarrow{\ZZ_p}} \to\pi_0^{\flat}R$.
%   % \end{itemize}
% \end{proof}
  % As a consequence of \Cref{rmk:splitting-comm} we learn that splittings are natural in commutative algebra maps.
%% \begin{rmk}
%%   Let $R \in \Alg(\Sp^{B\Z,u})$ and
%%   let $S(R)$ denote the Stone topological space associated to
%%   the boolean algebra of central idempotents in $\pi_*(R)$.
%%   The $\Z$-action on $R$ induces one on $S(R)$.
%%   Although we will not use it,
%%   we note that a splitting of the $\Z$-action on $R$ is equivalent to a
%%   $\Z$-equivariant continuous map
%%   $\overrightarrow{\ZZ_p} \to S(R)$.
%% \end{rmk}

\begin{lem} \label{lem:res-split}
  Let $\CC$ be a stable, presentably symmetric monoidal category
  and suppose we are given an $R \in \Alg(\CC^{B\Z,u})$.
  If the $\Z$-action on $R$ is split, 
  then the action of $p^k\Z \subseteq \Z$ on $R$ is also split.    
\end{lem}

\begin{proof}
  After restricting to $p^k\Z$ the original splitting of $R$
  becomes a lift of $R$ to a $\Z$-equivariant $\W\LCF{\Z_p}$-algebra
  where the $\Z$-action on $\W\LCF{\Z_p}$ is via the map $+p^j : \Z_p \to \Z_p$.
  The desired splitting of $R$ with the restricted action
  is now obtained by restriction along
  the map of commutative algebras associated to the $\Z$-equivariant map of Stone spaces
  \[  \lfloor -/p^k \rfloor : (\Z_p, +p^k) \to (\Z_p, +1). \qedhere \]
\end{proof}

% the natural setting to say this is finitary additive invariants from a p-complete stable infty-2 category
\begin{lem} \label{lem:extract-stone}
  Let $R \in \Alg(\Sp)$, and
  let $S$ be a Stone topological space.
  There is a natural isomorphism
  \[ K(\W(\LCF{S}) \otimes R) \cong \W(\LCF{S}) \otimes K(R). \]
\end{lem}

\begin{proof}
  Write $S$ as a cofiltered limit $\varprojlim S_\alpha$
  of finite discrete spaces $S_\alpha$.
  Using the fact that each of the functors $K(-)$, $\W(-)$ and $- \otimes R$
  commute with filterd colimits and finite products
  (for $\W(-)$ see \cite[Prop. 2.2, Lem. 2.10]{chromaticNSTZ})
  the composite $K(\W(-) \otimes R)$ does as well.
  We now construct a chain of isomorphisms 
  \begin{align*}
    K(\W(\LCF{S}) &\otimes R)
    \cong K\left(  \W\left( \varinjlim_{\alpha} \F_p^{\times S_\alpha} \right) \otimes R \right) 
    \cong \varinjlim_{\alpha}  K\left(  \W\left( \F_p \right) \otimes R \right)^{\times S_\alpha} \\
    &\cong \left( \varinjlim_{\alpha} \Ss^{\times S_\alpha} \right) \otimes K\left( \Ss \otimes R \right) 
    \cong \left( \varinjlim_{\alpha}  \W\left( \F_p \right)^{\times S_\alpha} \right) \otimes K(R) \\
    &\cong \W\left( \varinjlim_{\alpha} \F_p^{\times S_\alpha} \right)\otimes K(R) 
    \cong \W \LCF{S} \otimes K(R). 
  \end{align*}
\end{proof}

\begin{lem} \label{lem:extract-stone2}
  Let $R \in \Alg(\Sp_{T(n)})$ and 
  Let $S$ be a Stone topological space.
  There is a natural isomorphism
  \[ L_{T(n+1)}K(L_{T(n)}(\W(\LCF{S}) \otimes R)) \cong L_{T(n+1)}(\W(\LCF{S}) \otimes K(R)). \]
\end{lem}

\begin{proof}
  As $R$ is $T(n)$-local, the map
  $\W(\LCF{S}) \otimes R \to L_{T(n)}(\W(\LCF{S}) \otimes R)$
  is a $(T(n) \oplus T(n+1))$-local isomorphism and
  therefore we have a natural isomorphism  
  \[ L_{T(n+1)}K(L_{T(n)}(\W(\LCF{S}) \otimes R)) \cong L_{T(n+1)}K(\W(\LCF{S}) \otimes R) \]
  by the purity theorem of \cite{LMMT}.
  The lemma now follows from \Cref{lem:extract-stone}.  
\end{proof}

\begin{lem}\label{lem:assembly}
  Let $R \in \Alg(\Sp_{T(n)}^{B\Z,u})$ and
  suppose that the $\Z$-action on $R$ is $T(n)$-locally split.
  The coassembly map  
  \[ L_{T(n+1)}K(R^{h\ZZ} ) \to L_{T(n+1)}K(R)^{h\ZZ}\]
  is an isomorphism.
\end{lem}

\begin{proof}
  Let $Q \coloneqq R^{h\Z}$. 
  Using \Cref{prop:unipotent_SW} the splitting of the $\Z$-action gives us a $\Z$-equivariant  isomorphism
  \[ R \cong L_{T(n)}( \W\LCF{\overrightarrow{\ZZ_p}} \otimes Q ). \]
  In order to prove the lemma we must show that the $B\Z^{\lhd}$ diagram 
  \[ L_{T(n+1)}K(Q) \to L_{T(n+1)}K(L_{T(n)}( \W\LCF{\overrightarrow{\ZZ_p}} \otimes Q) \]
  is a limit cone.
  Applying \Cref{lem:extract-stone2} we can rewrite this as the diagram
  \[ L_{T(n+1)}K(Q) \to L_{T(n+1)}(\W\LCF{\overrightarrow{\ZZ_p}} \otimes K(Q)) \]
  which is a limit cone by \Cref{prop:unipotent_SW} (3).
\end{proof}

The following lemma will be useful in showing extensions are $T(n)$-locally split:

\begin{lem} \label{lem:intermediate-split}
    Let $\CC$ be a $p$-complete presentably symmetric monoidal stable category and let $A \to B$ be a map in $\CAlg(\CC)$. Suppose we have an intermediate map $A \to C \to D \to B$, where $C \to D$ is a pro-$\Z_p$-Galois extension. 
    
    Then if we restrict the $\Z_p$-action on $D$ to a $\Z$-action via a topological generator, the action on $D\otimes_AB$ is locally unipotent and the map $C\otimes_AB \to D\otimes_AB$ is split.
\end{lem}

\begin{proof}
Note that by replacing $\CC$ with $\Mod_{\CC}(A)$, we can assume that $A$ is the unit. By \Cref{rmk:splitting-comm}, Once we know the result for $B = D$, we learn it in general because of the map $D \to B$.

Thus, we want to show that $C\otimes D \to D\otimes D$ is split. To see this, we use the fact that 

$$\otimes_AB \implies \otimes_C B$$
We note that there are isomorphisms $D\otimes_AB \cong D\otimes_AC\otimes_CD$  



Unrolling definitions we see that it will suffice to prove that
  the $\Z$-action on
  \[ \Ss_{T(n)}\iwa{\infty}{n} \otimes \Ss_{T(n)}\iwa{\infty}{n} \otimes_{\Ss_{T(n)}\iwa{j}{n}} A \]
  coming from the Galois extension $\Ss_{T(n)}\iwa{j}{n+1} \to \Ss_{T(n)}\iwa{\infty}{n}$ is $T(n)$-locally split. As we have now moved to the commutative setting, we may use \Cref{rmk:splitting-comm} to conclude that it will suffice to produce this splitting in the case $A=\Ss_{T(n)}\iwa{j}{n}$. The $\Z$-action on $\Ss_{T(n)}\iwa{\infty}{n} \otimes \Ss_{T(n)}\iwa{\infty}{n}$ that we wish to split is the restriction to $p^j\Z$ of the full $\Z$-action on second factor and by \Cref{lem:res-split} it will suffice to split the latter action. 

  Using the fact that the cyclotomic extensions are Galois we have an
  isomorphism of $\Z$-equivariant $\Ss_{T(n)}\iwa{j}{n+1}$-algebras
  \[\Ss_{T(n)}\iwa{\infty}{n} \otimes \Ss_{T(n)}\iwa{\infty}{n} \cong \Ss_{T(n)}\iwa{\infty}{n} \otimes \W\LCF{\overrightarrow{\ZZ_p}}. \]
\end{proof}





